Split-NER: Named Entity Recognition via Two Question-Answering-based Classifications

In this work, we address the NER problem by splitting it into two logical sub-tasks: (1) Span Detection which simply extracts entity mention spans irrespective of entity type; (2) Span Classification which classifies the spans into their entity types. Further, we formulate both sub-tasks as question-answering (QA) problems and produce two leaner models which can be optimized separately for each sub-task. Experiments with four cross-domain datasets demonstrate that this two-step approach is both effective and time efficient. Our system, SplitNER outperforms baselines on OntoNotes5.0, WNUT17 and a cybersecurity dataset and gives on-par performance on BioNLP13CG. In all cases, it achieves a significant reduction in training time compared to its QA baseline counterpart. The effectiveness of our system stems from fine-tuning the BERT model twice, separately for span detection and classification. The source code can be found at https://github.com/c3sr/split-ner.

==> background.tex <==
Before diving into our pipelined framework, we start by re-implementing a standard single-model QA-based NER system over the BERT-base architecture (called \bertqa{} henceafter), which is similar to the MRC framework~\cite{li2020MRC}. 
In this setup, the model is fed a query specifying the target entity followed by the input sentence (e.g., \textit{``Where is \texttt{person} in the text? Emily lives in United States"}). 
The model is trained to understand the entity semantics from the query and output the corresponding mention spans from the sentence. 
Each token in the input sentence is classified into one of the four classes, \texttt{B} (begin), \texttt{I} (intermediate), \texttt{E} (end) and \texttt{O} (none), following the \texttt{BIOE} tagging scheme. 
Since each input asks for only one entity type, the BIOE classes are sufficient for NER.
We call this as the \bertqa{} model and train it on four different corpora (Table \ref{tab:datasets_summary}). 
Looking at the model predictions, we find that:
% (1) Mentions of same entity type can occur in diverse linguistic contexts; and (2) Mentions belonging to different entity types can occur in very similar linguistic contexts.
\begin{enumerate}[topsep=2pt,itemsep=1pt,parsep=1pt]
    \item Mentions of same entity type can occur in diverse linguistic contexts.
    \item Mentions belonging to different entity types can occur in very similar linguistic contexts.
\end{enumerate}

Table \ref{tab:findings} gives some examples of these cases. These findings reveal that we don't need entity-specific extraction rules, and the task of extracting a mention span can be decoupled from the task of classifying it into an entity type. 
\begin{table}[htbp]
\centering
\begin{small}
\begin{tabular}{l}\toprule
 Examples of same entity appearing in different contexts \\\midrule
% \textit{Investors were confident after watching success of \textcolor{blue}{Musk} in \textcolor{red}{Tesla}} \\
    \textit{People say \textcolor{blue}{Musk} and \textcolor{red}{Tesla} have a lot in common ...} \\
    \textit{With \textcolor{blue}{Musk}, \textcolor{red}{Tesla} is bound to have a promising future.} \\
    \textit{\textcolor{blue}{Musk} announced \textcolor{red}{Tesla's} new model ...} \\
     \textit{\textcolor{blue}{Musk's} \textcolor{red}{Tesla} has features not seen elsewhere.} \\
    \textit{The discussion was moderated by \textcolor{red}{Tesla's} \textcolor{blue}{Elon Musk}.} \\ \midrule \midrule
Examples of different entities in similar contexts \\ \midrule
\textit{Why do so many kids in \textcolor{magenta}{Digimon} wear gloves?} \\
\textit{Why do so many people in \textcolor{green}{Switzerland} speak German?} \\
 \textit{\textcolor{red}{Tesla} %[\texttt{Org}] 
 is bound to have a promising future with \textcolor{blue}{Musk}.} \\ %[\texttt{Person}].} \\
 \textit{\textcolor{blue}{Musk} %[\texttt{Person}] 
 is bound to have a promising future with \textcolor{red}{Tesla}.} %[\texttt{Org}].} 
 \\ \bottomrule
\end{tabular}
\caption{Examples showing that mention span detection and entity classification can be treated as independent tasks. Entity types are color-coded as \textcolor{blue}{\type{Person}}, \textcolor{red}{\type{Org}}, \textcolor{magenta}{\type{Product}} and \textcolor{green}{\type{Location}}.}
    \label{tab:findings}
\end{small}
\end{table}
%
Hence, we propose a two-stage pipelined system, \modelname{},  which has independent dedicated modules focusing on mention span detection and entity classification separately. 
This gives us the flexibility to design models tailor-made to cater to the needs of the individual sub-tasks.


==> loss.tex <==
As detailed earlier, Cross Entropy is an accuracy-oriented objective while during evaluation, we calculate the F1-Score. This difference can lead to sub-optimal model training. To counteract, \citet{li2019dice} make use of S{\o}rensen-Dice coefficient(DSC)\cite{sorensen1948method, dice1945measures} and Tversky index\cite{tversky1977features} which are F-Score oriented statistics. Given sets $A$ and $B$, DSC is used to gauge similarity among two sets and is defined as,
\begin{equation}
\label{eq:dsc_set}
    DSC(A, B) = \frac{2\ \vert A \cap B \vert}{\vert A \vert + \vert B \vert}
\end{equation}
Consider $A$ as set of all positive samples predicted by a model and $B$ as set of all ground truth positives. Then, by definition of true positive ($TP$), false positive ($FP$) and false negative ($FN$) from Section \ref{sec:evaluation_metrics}, we have,
\begin{equation}
\label{eq:dsc_tp}
    TP = \vert A \cap B \vert
\end{equation}
\begin{equation}
\label{eq:dsc_a}
    \vert A \vert = TP + FP
\end{equation}'
\begin{equation}
\label{eq:dsc_b}
    \vert B \vert = TP + FN
\end{equation}
Using Equations \ref{eq:dsc_tp}, \ref{eq:dsc_a} and \ref{eq:dsc_b}, in Equation \ref{eq:dsc_set}, we get,
\begin{equation}
\label{eq:dsc_as_f1}
     DSC(A, B) = \frac{2TP}{2TP + FP + FN} = \frac{2\ \frac{TP}{TP + FN}\ \frac{TP}{TP + FP}}{\frac{TP}{TP + FN} + \frac{TP}{TP + FP}} = \frac{2\ Precision \times Recall}{Precision + Recall} = F1
\end{equation}

The dice coefficient gives equal importance to false-positives and false-negatives at training time and is more immune to data-imbalance issues\cite{sudre2017generalised, shen2018influence, kodym2018segmentation}. The above formulation (Equation \ref{eq:dsc_as_f1}) shows its equivalence to F1-score thus removing the discrepancy among training and evaluation metrics. From Equation \ref{eq:dsc_set}, for an individual sample $x_i$, dice coefficient is defined as,
\begin{equation}
\label{eq:dsc_per_sample}
    DSC(x_i) = \frac{2p_{i1}y_{i1} + \gamma}{p_{i1} + y_{i1} + \gamma}
\end{equation}
where $\gamma$ is the smoothing parameter. Then over all samples, from Equation \ref{eq:dsc_per_sample}, dice loss (DL) is defined in Equation \ref{eq:dice_loss} as:
\begin{equation}
\label{eq:dice_loss}
    DL = 1 - \frac{2\sum_i{p_{i1}y_{i1}} + \gamma}{\sum_i{p_{i1}} + \sum_i{y_{i1}} + \gamma}
\end{equation}


==> training_efficiency.tex <==
Owing to its design, the \bertqa{} system %described in Section~\ref{sec:background}
essentially creates an input sample for each entity type and sentence pair. Thus, for a dataset with \textit{N} sentences and $|\mathcal{T}|$ entity types, the overall dataset size becomes \textit{N} $\times$ $|\mathcal{T}|$. 
This is a massive blow-up and, the model incurs a heavy latency for large datasets with many entity types.

Our system avoids the inefficiency by training two light-weight models. 
It also uses a QA setup but minimizes the redundant inputs. 
\spandetect{} asks one question for each input sentence to identify all required mentions, so the input size is $N$ for a dataset with $N$ sentences. 
\spanclass{} queries once for each mention span in a sentence, so the overall data size becomes \textit{N} $\times$ \textit{m} where \textit{m} is the average number of mentions in sentences. Note that \textit{m} is much smaller than $|\mathcal{T}|$.
For \data{OntoNotes5.0}, \bertqa{} generates $18$ queries for each sentence. 
\modelname{} would query once in \spandetect{} and $1.36$ times on average in \spanclass{} (see Table \ref{tab:datasets_summary}), providing a significant time efficiency. 


